Length Scales and Turbulent Properties of Magnetic Fields in Simulated Galaxy Clusters

Additional physics beyond standard hydrodynamics is needed to fully model the intracluster medium (ICM); however, as we move to more sophisticated models, it is important to consider the role of magnetic fields and the way the fluid approximation breaks down. This paper represents a first step towards developing a self-consistent model of the ICM by characterizing the statistical properties of magnetic fields in cosmological simulations of galaxy clusters. We find that plasma conditions are largely homogeneous across a range of cluster masses and relaxation states. We also find that the magnetic field length scales are resolution dependent and not based on any particular physical process. Energy transfer mechanisms and scales are also identified, and imply the existence of small scale dynamo action. The scales of the small scale dynamo are resolution limited and driven by numerical resistivity and viscosity.

==> an_scales.tex <==

\subsection{Analytic Scales}
\label{sec:an_scales}
As discussed previously, magnetic field-mediated particle interactions allow
the ICM to function as a fluid at large scales, but at smaller scales 
this assumption breaks down. In this section we examine characteristic
length and time scales in the intracluster medium that are related to
the magnetic field and to particle interactions. 

Whether the fluid approximation is valid for a given simulation is
determined by the ratio of the physical grid scale to the scale of interaction
that governs the behavior of the plasma.
In this section, we examine relevant plasma interaction
scales, comparing them to the grid scales in our simulations. These calculations
are critical to determining whether there are important physical processes
missing from our methodology that may impact our results. 

All following analysis is done by finding the total fraction of gas mass at a
given value of the quantity being examined, for a virial radius-sized
sphere.  Several important physical scales are shown in
Figure~\ref{fig:scales}, which was also discussed in the previous section.

We first examine the electron mean free path, defined as

    \begin{equation}
      \lambda_e = \frac{3^{3/2}(kT)^2}{4\pi^{1/2}n_e e^4 \ln \Lambda}
    \end{equation}
    
where $n_e$ is the electron number density and $\ln \Lambda$ is the Coulomb 
logorithm \citep{1965pfig.book.....S}. This mean free path is the scale over which electrons and ions
interact collisionally within the plasma. In pure hydrodynamics this sets a
limit on the scale on which the fluid approximation is valid in our
simulations (i.e., the spatial resolution of the simulation must be
substantially larger than this quantity).  Here we find that the mean free path is typically tens to
hundreds of kiloparsecs (top row) and is comparable to, and often
exceeds, the local 
cell size in our cosmological simulations (bottom row). Magnetic
fields will shorten the mean free path, however, as particle-particle
interactions are much more common in some directions along field
lines.  This makes the fluid
approximation still somewhat reasonable \citep{2011ASL.....4..204B},
although the reasonableness of the assumption depends somewhat on the tangledness of the magnetic
field on  scales comparable to the local simulation cell size.

Next, we show Debye Length, defined as

    \begin{equation}
      {L_D}^{-2} = \frac{4\pi e^2}{kT}(n_e+{Z_i}^2n_i)=\frac{8\pi e^2}{kT}n
    \end{equation}

where $n_i$ is the ion density. This is a measure of the length outside of
which charges are electrically screened. At length scales approaching the Debye length
a fully kinetic simulation is typically needed. In our cosmological simulations, however, the Debye length
is always many many orders of magnitude smaller than the cell size, indicating
that we are safe in our assumption that the plasma can be treated as a neutral
continuous field.

The proton gyroradius refers to the radius at which protons gyrate around a magnetic
field, and is defined by

    \begin{equation}
      \rho = \frac{v_{th}}{\Omega_i}~.
    \end{equation}

where $v_{th}$ is the thermal velocity and $\Omega=eB/m_p c$ is the proton 
gyrofrequency.  The proton gyroradius is typically quite small -- 
$\sim10^{-10}$~kpc -- and turns over quickly at smaller values and
slowly for larger values (note that the electron gyroradius is
generally substantially smaller than the proton gyroradius). The value 
becomes large and turns over slowly due to 
regions in the outskirts of the cluster where there is a very small magnetic
field.  

The electron equilibration time scale indicates how quickly the plasma can 
be considered to be in a thermalized state, where T$_e = $T$_{ion}$,
if the electron-ion collisions are dominated
by Coulomb interactions.  This scale is defined as:

    \begin{equation}
      t_{eq} = \frac{\lambda_e}{v_{th}}.
    \end{equation}

where $\lambda_e$ is the electron mean free path and v$_{th}$ is the
mean electron velocity of electrons at temperature T$_e$.
The electron equilibration time is short compared to the age of the cluster 
($t_{eq}\sim 10^6 - 10^8$~yr), and generally substantially smaller
than the local grid's Courant time (i.e., the time step taken by the
simulation in a given grid cell).
Additionally, Coulomb collisions are likely not the dominant interaction 
mechanism due to the presence of magnetic fields, as discussed previously.

Across all measures in Figure~\ref{fig:scales}, the clusters are
qualitatively similar to each other.  The 
distributions of each quantity do not deviate by much more than an order of magnitude across
clusters at a given value of that quantity, except in cases where low values are dominated by a lack
of magnetic field amplification in cluster outskirts. 


